Investor Emotions and Earnings Announcements

Armed with a decade of social media data, I explore the impact of investor emotions on earnings announcements. In particular, I test whether the emotional content of firm-specific messages posted on social media just prior to a firm's earnings announcement predicts its earnings and announcement returns. I find that investors are typically excited about firms that end up exceeding expectations, yet their enthusiasm results in lower announcement returns. Specifically, a standard deviation increase in excitement is associated with an 7.8 basis points lower announcement return, which translates into an approximately -5.8% annualized loss. My findings confirm that emotions and market dynamics are closely related and highlight the importance of considering investor emotions when assessing a firm's short-term value.

==> Tables/dictionaries.tex <==
\begin{table}[!h] \centering 
\footnotesize 
\caption{Dictionaries for Training Data}\label{tab:dictionaries}
\begin{tabular}{ll}
Word List & \# of Entries \\ \hline
& \\[\dimexpr-\normalbaselineskip+2pt]
\multicolumn{2}{l}{\textbf{Panel A: Emotions}} \\ 
& \\[\dimexpr-\normalbaselineskip+2pt]
Happy & 553 \\
Fear & 412 \\
Disgust & 325 \\
Sad & 288 \\
Surprise & 195 \\
Anger & 189 \\
Happy Emojis \& Emoticons & 143 \\
Sad Emojis \& Emoticons & 63 \\
Anger Emojis \& Emoticons & 39 \\
Fear Emojis \& Emoticons & 22 \\
Surprise Emojis \& Emoticons & 12 \\
Disgust Emojis \& Emoticons & 9 \\
& \\[\dimexpr-\normalbaselineskip+2pt]
\multicolumn{2}{l}{\textbf{Panel B: Information}} \\
& \\[\dimexpr-\normalbaselineskip+2pt]
Finance & 270 \\
Earnings & 84 \\ \hline \hline 
\end{tabular}
\end{table}

==> Tables/doc_similarity.tex <==
\begin{table}[htbp]\centering
\footnotesize 
\caption{Document Similarity}\label{tab:doc_sim}
\begin{threeparttable}
\begin{tabular}[l]{lp{0.7in}p{0.5in}p{0.7in}p{0.5in}p{0.6in}p{0.5in}}
Document & Vocabulary & Total Words & Complexity & Diversity & Similarity (Tfidf) & Cluster \\ \hline 
Adventure & 7874 & 334889 & 13.6 & 0.009 & 0.83 & 3 \\
Editorial & 8586 & 331345 & 14.9 & 0.010 & 0.86 & 0 \\
Fiction & 8331 & 334313 & 14.4 & 0.010 & 0.83 & 3 \\
Genesis (English Web) & 2430 & 188666 & 5.6 & 0.014 & 0.78 & 3 \\
Government & 6864 & 396904 & 10.9 & 0.012 & 0.83 & 0 \\
Hobbies & 9911 & 441323 & 14.9 & 0.009 & 0.85 & 0 \\
Humor & 4613 & 109286 & 14.0 & 0.008 & 0.84 & 3 \\
Learned & 14201 & 1015908 & 14.1 & 0.012 & 0.83 & 0 \\
Mystery & 6135 & 274529 & 11.7 & 0.009 & 0.82 & 3 \\
Negative Tweets & 10647 & 321935 & 18.8 & 0.004 & 0.58 & 1 \\
New York Times: Editorials & 827 & 12584 & 7.4 & 0.012 & 0.80 & 0 \\
New York Times: Political & 801 & 12960 & 7.0 & 0.012 & 0.78 & 0 \\
New York Times: Sport & 845 & 12272 & 7.6 & 0.012 & 0.76 & 0 \\
News & 11880 & 543146 & 16.1 & 0.010 & 0.85 & 0 \\
Positive Tweets & 13175 & 373440 & 21.6 & 0.004 & 0.49 & 1 \\
Religion & 5780 & 207979 & 12.7 & 0.011 & 0.85 & 0 \\
Reviews & 7705 & 218527 & 16.5 & 0.010 & 0.85 & 0 \\
Romance & 7500 & 335805 & 12.9 & 0.008 & 0.81 & 3 \\
Science Fiction & 2959 & 72153 & 11.0 & 0.009 & 0.82 & 3 \\
StockTwits Messages & 31114 & 7569605 & 11.3 & 0.005 & 0.71 & 1 \\
Times: National Affairs & 867 & 12972 & 7.6 & 0.011 & 0.77 & 0 \\
Tweets & 19045 & 2450175 & 12.2 & 0.006 & 0.34 & 2 \\
Twitter: Training Data & 34099 & 7759529 & 12.2 & 0.007 & 0.69 & 1 \\
Wall Street Journal: Financial & 765 & 12245 & 6.9 & 0.011 & 0.73 & 0 \\
Wall Street Journal: Reviews & 925 & 13043 & 8.1 & 0.013 & 0.80 & 0 \\
Washington Post: Cultural & 817 & 12407 & 7.3 & 0.015 & 0.79 & 0 \\ \hline \hline 
\end{tabular}
\begin{tablenotes}
\footnotesize
\item We define $\text{Complexity} = \frac{\text{Vocabulary}}{\sqrt{Total Words}}$ and Diversity = $\sum_{n=0}^{k} \Big(\frac{\# \text{of occurences word}_n}{Total Words}\Big)^2$ for each word n in the dictionary.
\end{tablenotes}
\end{threeparttable}
\end{table}

==> Tables/gbt.tex <==
\begin{table}[htbp]\centering
\footnotesize 
\begin{threeparttable}
\caption{Predictive Power of Social Media Emotions \& Opinion \label{tab:gbt}}
\begin{tabular}{p{4in}p{1in}p{1in}}
Feature set & Statistic &/ Firm Returns \\ \hline
& & \\[\dimexpr-\normalbaselineskip+2pt]
One & Mean & 0.855 \\
 & Std. Dev. & 0.040 \\
 & & \\[\dimexpr-\normalbaselineskip+2pt]
Two & Mean & 0.903 \\
& Std. Dev. & 0.041 \\ \hline 
 & & \\[\dimexpr-\normalbaselineskip+2pt]
& p-value  & 0.0155 \\ \hline \hline 
\end{tabular}
\begin{tablenotes}
\footnotesize  
\item We train and validate a GBT model on 2010-2018 data, and test it on 2019 data. We use 10-fold CV on the training data (each evaluated on the test data) to get mean and standard deviations. GBT parameters: 1000 trees, early stopping of 50 rounds, depth of 2, learning rate of 0.05.  %We report the two-sided test (p-value) for the null hypothesis that two models have identical expected values.
\end{tablenotes}
\end{threeparttable}
\end{table}

==> Tables/trading_strategy.tex <==
\begin{table}[htbp]\centering
\footnotesize 
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{threeparttable}
\caption{Trading Strategy \label{tab:trading_strategy}}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{1}{c}{Portfolio}&\multicolumn{1}{c}{Long}&\multicolumn{1}{c}{ Short}&\multicolumn{1}{c}{Portfolio}&\multicolumn{1}{c}{ Long}&\multicolumn{1}{c}{ Short}\\
\hline
&             &           &           &            &           &    \\[\dimexpr-\normalbaselineskip+2pt]
Mkt-RF              &      0.6404\sym{***}&      0.7062\sym{***}&      0.5743\sym{***}&      0.7669\sym{***}&      0.8275\sym{***}&      0.7166\sym{***}\\
                    &    (0.0528)         &    (0.0804)         &    (0.0620)         &    (0.0762)         &    (0.1170)         &    (0.0884)         \\
&             &           &           &            &           &    \\[\dimexpr-\normalbaselineskip+2pt]
SMB                 &      0.3948\sym{***}&      0.3825\sym{***}&      0.4146\sym{***}&      0.5498\sym{***}&      0.5283\sym{***}&      0.5793\sym{***}\\
                    &    (0.0808)         &    (0.1097)         &    (0.1156)         &    (0.1025)         &    (0.1407)         &    (0.1540)         \\
&             &           &           &            &           &    \\[\dimexpr-\normalbaselineskip+2pt]
HML                 &      0.0334         &      0.0915         &     -0.0105         &      0.1559         &      0.2392         &      0.0945         \\
                    &    (0.0824)         &    (0.1270)         &    (0.1184)         &    (0.1045)         &    (0.1648)         &    (0.1543)         \\
&             &           &           &            &           &    \\[\dimexpr-\normalbaselineskip+2pt]
Mom                 &     -0.2153\sym{**} &     -0.4337\sym{***}&      0.0175         &     -0.2516\sym{**} &     -0.4921\sym{**} &      0.0155         \\
                    &    (0.0906)         &    (0.1475)         &    (0.1031)         &    (0.1220)         &    (0.2007)         &    (0.1389)         \\
&             &           &           &            &           &    \\[\dimexpr-\normalbaselineskip+2pt]
Constant            &      0.0235         &     -0.1970\sym{***}&      0.2602\sym{***}&      0.0837\sym{*}  &     -0.1979\sym{***}&      0.3845\sym{***}\\
                    &    (0.0390)         &    (0.0573)         &    (0.0551)         &    (0.0501)         &    (0.0727)         &    (0.0716)         \\
\hline
&             &           &           &            &           &    \\[\dimexpr-\normalbaselineskip+2pt]
Sample & Entire & Entire & Entire & $\ge 2013$ & $\ge 2013$ & $\ge 2013$ \\
Observations        &   2516         &   2516         &   2516         &   1762         &   1762         &   1762         \\
$R^2$               &      0.1210         &      0.0777         &      0.0524         &      0.1168         &      0.0766         &      0.0510         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\footnotesize 
\item Notes:  Robust standard errors in parentheses. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). 
\end{tablenotes}
\end{threeparttable}
\end{table}

